Optimizing BLE-Like Neighbor Discovery

Neighbor discovery (ND) protocols are used for establishing a first contact between multiple wireless devices. The energy consumption and discovery latency of this procedure are determined by the parametrization of the protocol. In most existing protocols, reception and transmission are temporally coupled. Such schemes are referred to as \textit{slotted}, for which the problem of finding optimized parametrizations has been studied thoroughly in the literature. However, slotted approaches are not efficient in applications in which new devices join the network gradually and only the joining devices and a master node need to run the ND protocol simultaneously. For example, this is typically the case in IoT scenarios or Bluetooth Low Energy (BLE) piconets. Here, protocols in which packets are transmitted with periodic intervals (PI) can achieve significantly lower worst-case latencies than slotted ones. For this class of protocols, optimal parameter values remain unknown. To address this, we propose an optimization framework for PI-based BLE-like protocols, which translates any specified duty-cycle (and therefore energy budget) into a set of optimized parameter values. We show that the parametrizations resulting from one variant of our proposed scheme are optimal when one receiver discovers one transmitter, and no other parametrization or ND protocol - neither slotted nor slotless - can guarantee lower discovery latencies for a given duty-cycle in this scenario. Since the resulting protocol utilizes the channel more aggressively than other ND protocols, beacons will collide more frequently. Hence, due to collisions, the rate of successful discoveries gracefully decreases for larger numbers of devices discovering each other simultaneously. We also propose a scheme for configuring the BLE protocol (and not just BLE-\textit{like} protocols).

==> sections/optimality.tex <==
\section{Hypothsis of Optimality}
\label{sec:optimality}
We hypothesize that the parameter values returned by the $PI-0M$ scheme are optimal for the corresponding duty cycle. This hypothesis is strengthened by the results returned by an exhaustive search over the parameter space, modulo a certain discretization. The discovery latencies computed using parameter values obtained from such an exhaustive search are always greater than the discovery latencies resulting from the parameter values returned by our proposed framework. Note that such an exhaustive search can never replace a framework like the one we are proposing because it always relies on a discretization and hence certain parameterizations are not explored.

Equation~\ref{eq:pi0MMopt} gives an optimal value of $M$, which is in general a fractional number that has to be rounded to the next integer value. More specifically, our hypothesis is that parameterizations for which Equation 6 returns an integer value of $M$ are optimal (viz., no other parameterizations will lead to a shorter discovery latency). Parameterizations for which Equation~\ref{eq:pi0MMopt} returns a fractional value of $M$ – and hence $M$ is rounded to the next integer value – are not necessarily optimal, but for all practical purposes the resulting discovery latency is almost equal to the discovery latency resulting from an optimal parameterization. 

For the exhaustive search over the parameter space, we considered all values of $T_a$ and $T_s$ between $\SI{10}{ms}$ and $\SI{5}{s}$ in discrete steps of $\SI{10}{ms}$, whereas all values of $d_s$ between $\SI{10}{ms}$ and $T_s$ were considered with the same discretization. To compute the discovery latencies, we used a generic model for PI-based protocols from the literature~\cite{kindt:15}. We have assumed a packet length of $\SI{30}{bytes}$. Whenever the corresponding duty-cycle lay within a reasonable range of $\SI{0.1}{\percent}$ to $\SI{10}{\percent}$, we also computed the latency achieved by the $PI-0M$ scheme for this duty-cycle. For all examined values of $T_a$, $T_s$ and $d_s$, the latencies obtained for $PI-0M$ were lower than the ones obtained for these parameter values. The smallest difference between any latency examined during the search and the corresponding latency of the $PI-0M$ scheme has been $\SI{165}{ms}$. This strengthens our hypothesis and suggests that future work should further study the optimality of these values. 
